Combining Program Analysis and Statistical Language Model for Code Statement Completion

Automatic code completion helps improve developers' productivity in their programming tasks. A program contains instructions expressed via code statements, which are considered as the basic units of program execution. In this paper, we introduce AutoSC, which combines program analysis and the principle of software naturalness to fill in a partially completed statement. AutoSC benefits from the strengths of both directions, in which the completed code statement is both frequent and valid. AutoSC is first trained on a large code corpus to derive the templates of candidate statements. Then, it uses program analysis to validate and concretize the templates into syntactically and type-valid candidate statements. Finally, these candidates are ranked by using a language model trained on the lexical form of the source code in the code corpus. Our empirical evaluation on the large datasets of real-world projects shows that AutoSC achieves 38.9-41.3% top-1 accuracy and 48.2-50.1% top-5 accuracy in statement completion. It also outperforms a state-of-the-art approach from 9X-69X in top-1 accuracy.

==> RQ1_SC_within.tex <==
\begin{table}[]
\centering
\caption{SC Accuracy}
\label{RQ1_SC_within}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Project   & \begin{tabular}[c]{@{}l@{}}Rec.\\ Size\end{tabular}   & TOOL                                                    & \begin{tabular}[c]{@{}l@{}}Lexical \\ n-gram\end{tabular} & \begin{tabular}[c]{@{}l@{}}Lexical\\ n-gram + PA\end{tabular} & \begin{tabular}[c]{@{}l@{}}Rel. \\ Improv.\end{tabular} \\ \hline
Ant       & \begin{tabular}[c]{@{}l@{}}Top 1\\ Top 5\end{tabular} & \begin{tabular}[c]{@{}l@{}}X\%\\ X\%\end{tabular} &                                                           &                                                               &                                                         \\ \hline
Batik     & \begin{tabular}[c]{@{}l@{}}Top 1\\ Top 5\end{tabular} & \begin{tabular}[c]{@{}l@{}}X\%\\ X\%\end{tabular}                                                        &                                                           &                                                               &                                                         \\ \hline
Cassandra & \begin{tabular}[c]{@{}l@{}}Top 1\\ Top 5\end{tabular} & \begin{tabular}[c]{@{}l@{}}X\%\\ X\%\end{tabular}                                                        &                                                           &                                                               &                                                         \\ \hline
Log4J     & \begin{tabular}[c]{@{}l@{}}Top 1\\ Top 5\end{tabular} & \begin{tabular}[c]{@{}l@{}}X\%\\ X\%\end{tabular}                                                        &                                                           &                                                               &                                                         \\ \hline
Lucene    & \begin{tabular}[c]{@{}l@{}}Top 1\\ Top 5\end{tabular} & \begin{tabular}[c]{@{}l@{}}X\%\\ X\%\end{tabular}                                                        &                                                           &                                                               &                                                         \\ \hline
Maven-2   & \begin{tabular}[c]{@{}l@{}}Top 1\\ Top 5\end{tabular} & \begin{tabular}[c]{@{}l@{}}X\%\\ X\%\end{tabular}                                                        &                                                           &                                                               &                                                         \\ \hline
Maven-3   & \begin{tabular}[c]{@{}l@{}}Top 1\\ Top 5\end{tabular} &  \begin{tabular}[c]{@{}l@{}}X\%\\ X\%\end{tabular}                                                       &                                                           &                                                               &                                                         \\ \hline
Xalan     & \begin{tabular}[c]{@{}l@{}}Top 1\\ Top 5\end{tabular} &  \begin{tabular}[c]{@{}l@{}}X\%\\ X\%\end{tabular}                                                       &                                                           &                                                               &                                                         \\ \hline
Xerces    & \begin{tabular}[c]{@{}l@{}}Top 1\\ Top 5\end{tabular} &  \begin{tabular}[c]{@{}l@{}}X\%\\ X\%\end{tabular}                                                       &                                                           &                                                               &                                                         \\ \hline
\end{tabular}
\end{table}

==> RQ1_next_stm.tex <==
\textbf{For \textit{SS}}, table \ref{RQ1_SC} shows that {\tool} outperforms the state-of-the-art approach~\cite{ase_17}. Specifically, the top-1 accuracy of {\tool} is relatively higher than PPC XXX--YYY\%. Meanwhile, {\tool} also achieved a much higher top-5 accuracy, XXX-YYY\% relatively. 

Analyzing the results, we found a reason that PPC achieved a low accuracy.  

\input{statement_suggestion}

==> background.tex <==
\subsection{Background}

\textbf{About different code token types}
\begin{table}[h]
\centering
\caption{Different token types in Java programming language}
\label{token_types}
\begin{tabular}{|l|l|}
\hline
Lexeme & Token Type \\ \hline
 & Identifier \\ \hline
 & Keyword \\ \hline
 & Literal \\ \hline
 & Separator \\ \hline
 & Operator \\ \hline
\end{tabular}
\end{table}
%https://docs.oracle.com/javase/specs/jls/se7/html/jls-3.html

\textbf{About Program Constraints}
Compiler's principle (Syntax, Type)



\textbf{About Statistical Language Model}

==> discussion.tex <==
\section{Discussion}

==> general_algo.tex <==
\subsection{{\tool} Algorithm}

In summary, {\tool} algorithm for statement completion with all
previously described steps is presented in Algorithm~\ref{algo}.

\begin{algorithm}[t]
\caption{{\tool}: Automated Statement Completion}	
\label{algo}
\begin{algorithmic}[1]
%$excodeLM$, $lexemesLM$
\Function {complete}{$partialCode$, $P$}
	\State $T = identifyTempls(partialCode, P)$ \Comment{Algo.~\ref{agl1}}
	\State $validCands = \emptyset$
	\ForAll {$cand \in T$}
		\If {$typeCheck(cand, partialCode)$}
			\State $validCands.adds(cand)$
		\EndIf
	\EndFor
	\State $V = findAccessiblelVars(partialCode,P)$
	\State $codeCands = concretize(validCands, V)$
	\State \textbf{return} $rank(codeCands, partialCode, \phi_{lexemes})$
\EndFunction
\end{algorithmic}
\end{algorithm}


==> ideas.tex <==
\subsection{Key Ideas and Approach Overview}
\label{keyideas-section}


==> motivation_backup.tex <==
%Method_ID: ASE19_METHOD_457020
\begin{figure}[t]
\begin{center}
\lstinputlisting[captionpos=b, basicstyle={\footnotesize\ttfamily}]{example.java}
%\lstinputlisting[captionpos=b]{example_img.java}
\vspace{-0.15in}
\caption{A partial method in Apache Ant}
\label{example1}
\end{center}
\end{figure}
%

For \textit{program analysis}, although the number of legal valid candidates for the next token is limited, the number of possible legal completed statements might be infinite. For the right side of the assignment at line 5, the legal next-token candidates include appropriate prefix operators (e.g., \texttt{++} and \texttt{--}), the open parenthesis, accessible fields, methods and local variables (e.g., \texttt{children} or \texttt{f}). There is infinite number of valid statements can be completed in this case, one possible legal suggestion is \texttt{f.toString().subString(3).} \texttt{toString().replace("hello", "").length();}.

%Meanwhile, most of code statement are not too complex, XXX\% statements do not composed by more than YYY code tokens.

%linking...

For \textit{language models}, which is leveraged on the idea that code is highly repetitive and predictable~\cite{prem_naturalness}, given a partial code statement, the next token can be suggested based on the frequency of code tokens. However, since code is strictly constrained by syntax and semantics (e.g., type), purely using statistical language models which are leveraged on the repetition of code could be faced with the problem of program constraint violations. For the example shown in figure \ref{example1}, the most likely tokens recommended for the right side of the assignment at line 5 includes: "\texttt{;}", "\texttt{(}", "\texttt{)}", or "\texttt{i}" which are extremely frequent in the code corpus. That induces syntax errors or \textit{use undeclared variable}.
%
%About the combination: PA and statistical LMs complement each other
%How to link...???
%

Hence, \textit{combining PA and LM could exploit the strengths of both of them in predicting the next token}. In particular, \textit{PA} could be used to limit the legal candidates for the next token, then \textit{LM}s could be used to apply the principal of code repetition on these legal tokens. For example, to suggest the next token of the statement at line 5, one could use \textit{LM} to identify the likelihood of the legal candidates such as \texttt{children}, \texttt{parent} or \texttt{f}.
%
%For the example shown in figure \ref{example1}, the set of valid candidates for the next token includes local variables (e.g., \texttt{children}, \texttt{parent}, \texttt{f}, or \texttt{matches}), accessible fields and methods, appropriate operators (e.g., \texttt{++} or \texttt{--}), and the open parenthesis (100 valid candidates out of XXX unique tokens in the project). 
% TODO: temporary ranking numbers 
%
%

However, \textit{since the local variables are designed to be used locally, the usage regularity/pattern of these local variables could not be captured from the other methods/classes/projects}. For example, since there is no statement starting with "\texttt{int len = children}" or "\texttt{int len = f}", in the entire project, the variables \texttt{children} and \texttt{f} are both ranked very low, ZZZ out of 100 legal candidates of the next token. 
% 
%
Meanwhile, the pattern/template \texttt{VAR(int) = VAR(NodeList)} (such as \texttt{int size = nodes.getLength()}) appears in XXX methods, and the pattern/template \texttt{VAR(int) = VAR(NodeFilter)} is never applied in the project. 
%
%
As a result, for the example, the local variable having type \texttt{NodeList} should be more likely to be the next token than the variable having type \texttt{NodeFilter}. Moreover, there is only one local variable type \texttt{NodeList}, \texttt{children} which is the correct one, that can be identified by \textit{PA}. 
%
Hence, \textit{the usage regularity/pattern of the type of local variables could be captured better in suggesting the next token, by considering local variables without names which are identified using PA in a limited set of local variables}.

%
%For completed statements:

By combining \textit{PA} and \textit{LM} in predicting token by token, the number of resulting valid statements might be still extremely large. For this example, if for each step, 5 of most likely valid tokens are predicted, the number of completed legal statement candidates having at most 10 code tokens and is more than \textbf{5,000}, such as \texttt{int len = children.getLength();} and \texttt{int len = JavaCC.TASKDEF\_TYPE\_JAVACC;}
%Might need resulting statement here

Since the lexical form of the name of program elements (variables/methods/field/types), such as "\texttt{children}", "\texttt{get length}" or "\texttt{taskdff type javacc}", caries certain meaning that reflects the semantics role of the elements~\cite{???}, \textit{the lexical meaning of the resulting valid statement might be useful to identify the likelihood of the completed statements}. In figure \ref{example1}, the correct completed statement \texttt{int len = children.getLength();} should be ranked higher than \texttt{int len = JavaCC.TASKDEF\_TYPE\_JAVACC;}

%Since the lexical form of the name of program elements (variables/methods/field/types) caries certain meaning that reflects the semantics role of the elements, a LM based on the lexical form of the names in code can evaluate on the likelihood of the completed statements' meaning. In the example in figure \ref{example1}, the well-form candidates for the right side of the assignment containing words \texttt{length}, \texttt{size} or \texttt{len} should be ranked higher than ones containing words \texttt{version} or \texttt{top}.


\textbf{Observation}. A partial code statement/new statement should be completed/suggested token by token by combining program syntax and semantics constraints (\textit{PA}) and the principal of code repetition (\textit{LM}). In this process, for local variables, to capture better the code usage regularity/pattern, their type should be taken into account, rather than variables' name that could be determined by using \textit{PA}. Additionally, lexical meaning of legal completed statements also plays a crucial role in determining the likelihood of the compilations.

==> observation.tex <==
\subsection{Observations and Approach Motivation}


==> statement_suggestion.tex <==
\begin{table}[]
\centering
\caption{Next-statement Suggestion Accuracy}
\label{RQ1_SC}
\begin{tabular}{ll|llll}
\toprule
Project   & \begin{tabular}[c]{@{}l@{}}Rec.\\ Size\end{tabular}   & {\tool}                                                    &  PPC~\cite{ase_17} & \begin{tabular}[c]{@{}l@{}}Rel. \\ Improv.\end{tabular} \\ \hline
Ant       & \begin{tabular}[c]{@{}l@{}}Top 1\\ Top 5\end{tabular} & \begin{tabular}[c]{@{}l@{}} 8.5\%\\ 12.5\%\end{tabular} &\begin{tabular}[c]{@{}l@{}} 1.7\%\\ 4.1\%\end{tabular}				&                                                                                                                                                                          \\ \hline
Batik     & \begin{tabular}[c]{@{}l@{}}Top 1\\ Top 5\end{tabular} & \begin{tabular}[c]{@{}l@{}} 8.1\%\\ 11.8\%\end{tabular} &\begin{tabular}[c]{@{}l@{}} 3.9\%\\ 6.8\%\end{tabular}					&                                                                                                                                                                  \\ \hline
Cassandra & \begin{tabular}[c]{@{}l@{}}Top 1\\ Top 5\end{tabular} & \begin{tabular}[c]{@{}l@{}} 8.3\%\\ 12.7\%\end{tabular} & \begin{tabular}[c]{@{}l@{}} 2.5\%\\ 5.4\%\end{tabular}					&                                                                                                                                                                                 \\ \hline
Log4J     & \begin{tabular}[c]{@{}l@{}}Top 1\\ Top 5\end{tabular} & \begin{tabular}[c]{@{}l@{}} 7.9\%\\ 11.3\%\end{tabular} &				\begin{tabular}[c]{@{}l@{}} 0.9\%\\ 3.8\%\end{tabular}	&                                                                                                                                                                                \\ \hline
Lucene    & \begin{tabular}[c]{@{}l@{}}Top 1\\ Top 5\end{tabular} & \begin{tabular}[c]{@{}l@{}} X\%\\ X\%\end{tabular} &					\begin{tabular}[c]{@{}l@{}} 3.8\%\\ 5.9\%\end{tabular}&                                                                                                                                                                                   \\ \hline
Maven-2   & \begin{tabular}[c]{@{}l@{}}Top 1\\ Top 5\end{tabular} & \begin{tabular}[c]{@{}l@{}} X\%\\ X\%\end{tabular} &					\begin{tabular}[c]{@{}l@{}} 0.6\%\\ 3.1\%\end{tabular}&                                                                                                                                                                                   \\ \hline
Maven-3   & \begin{tabular}[c]{@{}l@{}}Top 1\\ Top 5\end{tabular} & \begin{tabular}[c]{@{}l@{}} X\%\\ X\%\end{tabular} &					\begin{tabular}[c]{@{}l@{}} 1.2\%\\ 4.7\%\end{tabular} &                                                                                                                                                                                   \\ \hline
Xalan     & \begin{tabular}[c]{@{}l@{}}Top 1\\ Top 5\end{tabular} &  \begin{tabular}[c]{@{}l@{}} X\%\\ X\%\end{tabular} &					\begin{tabular}[c]{@{}l@{}} 2.6\%\\ 5.2\%\end{tabular} &                                                                                                                                                                                   \\ \hline
Xerces    & \begin{tabular}[c]{@{}l@{}}Top 1\\ Top 5\end{tabular} &  \begin{tabular}[c]{@{}l@{}} X\%\\ X\%\end{tabular} &					\begin{tabular}[c]{@{}l@{}} 2.1\%\\ 5.5\%\end{tabular}&                                                                                                                                                                                   \\ \toprule
\end{tabular}
\end{table}


==> type_exploratory.tex <==

\begin{table*}[]
\centering
\caption{Data type contexts and the data type repetition of token in the being-predicted expressions}
\label{type_explore}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{Kind} & \multirow{2}{*}{Data type context} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Being-predicted\\ Expressions ($bes$)\end{tabular}} & \multicolumn{3}{l|}{$types(bes)$'s repetition} \\ \cline{4-6} 
 &  &  & \begin{tabular}[c]{@{}l@{}}Cross-\\ method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Cross\\ -file\end{tabular} & \begin{tabular}[c]{@{}l@{}}Cross-\\ project\end{tabular} \\ \hline
PrefixOp & OP{[}opName{]} & rightExpr & x & x & x \\ \hline
InfixOp & leftExp OP{[}oName{]} & rightExpr & x & x & x \\ \hline
Assignment & leftExp ASSIGN{[}assign{]} & rightExpr & x & x & x \\ \hline
Method call arguments & M\_A {[}T, mtName, argsCount, rtType{]} & arguments & x & x & x \\ \hline
Return expression & ReturnType & returnExpr & x & x & x \\ \hline
Control expression & ControlStatement & controlExpr & x & x & x \\ \hline
\end{tabular}%
}
\end{table*}

==> type_infer.tex <==
%\begin{table*}[]
%\centering
%\caption{Popular type inference rules}
%\label{type_infer}
%\begin{tabular}{|l|l|l|}
%\hline
%Kind                  & \textit{Excode} expression, $e$                    %         & Type,  $dt(e)$ \\ \hline
%Literal               & \code{LIT(T)}                           & \code{T} %              \\ \hline
%Variable              & \code{VAR(T)}                                 & \code{T}               \\ \hline
%Method call           & \code{{[}exp OP(access){]} CALL(O,m,c,RT)} & \code{RT}              \\ \hline
%Field access          & \code{{[}exp OP(access){]} FIELD(O,f,FT)}  & \code{FT}              \\ \hline
%Prefix     			 & \code{OP(prefixOp) expr}                  %    & \begin{tabular}[c]{@{}l@{}}$dt(expr)$, if $dt(expr)$ is not $Unknown$\\ $boolean$, if \code{OP(not)}\\$int$, otherwise\end{tabular}  \\ \hline
%Postfix			     & \code{expr OP(prefixOp)}                      & \begin{tabular}[c]{@{}l@{}}$dt(expr)$, if $dt(expr)$ is not $Unknown$\\ $int$, otherwise\end{tabular} \\ \hline
%Comparison infix      & \code{left OP(compareOp) right}              & \code{boolean}         \\ \hline
%Other infix 			  & \code{left OP(infixOp) right}                & $dt(right)$ \\ \hline
%Other infix 			  & \code{left OP(infixOp) right}                &    \begin{tabular}[c]{@{}l@{}}$dt(right)$, if $dt(right)$ is not $Unknown$\\ $dt(left)$, otherwise\end{tabular}\\ \hline
%\end{tabular}
%\end{table*}


\begin{algorithm}
\caption{Identifying \textit{excode} expression type}	
 \label{type_infer_algo}
\begin{algorithmic}[1]
\Function {dt}{$exp$}
	\If {$isVAR(exp) \lor isLIT(exp)$}
		\State \textbf{return} $type(exp)$
	\EndIf
	\If {$isComparison(exp)$}
		\State \textbf{return} $boolean$
	\EndIf
	\If {$isCALL(exp)$}
		\State $call=extractCall(exp)$
		\State \textbf{return} $rettype(call)$
	\EndIf
	\If {$isFIELD(exp)$}
		\State $field=extractField(exp)$
		\State \textbf{return} $fieldtype(field)$
	\EndIf
	\If {$isInfix(exp)$ } \Comment{Not comparison operators}
		\State $rightExpr=extractRightExp(exp)$
		\State \textbf{return} $dt(rightExpr)$
	\EndIf
	\State \textbf{return} $null$
\EndFunction
\end{algorithmic}
\end{algorithm}


==> type_rules.tex <==
%https://docs.oracle.com/javase/specs/jls/se7/html/jls-18.html
Beside syntax, code is restricted by the rules in data type, that restrict the data type of the being predicted tokens of the given excode sequence. For example, the left side of the assignment, \texttt{VAR[NodeList] ASSIGN[assign]}, restricts the type of the excode tokens in the right side.

Based on program syntax~\cite{java_syntax}, we define data type contexts of excode sequences and the corresponding being-predicted excode expressions in Tab. \ref{type_explore} (column 1--3).


%\begin{itemize}
%\item Operators: prefix and infix operators
%%(6 prefix, 19 infix, and 2 postfix operators)
%\item Assignments 
%%(16 assignment operators)
%\item Method call arguments
%\item Return expression
%\item Control expression (including if-, while-do-, do-while-, for-, for-each-, switch-case- statements)
%\end{itemize}

Theoretically, given a excode sequence $S$ having data type context $dc$, to identify all possible types for the next token, ones have to analyze entire the current project and all available libraries, which is an impractical task. 
%

Meanwhile, data type is designed for the purpose of reuse, the use of data type in the context can be repeated. To understand use of data type, we performed an exploratory investigate repetition of the tokens in the being predicted expressions. 
%
For a excode sequence $S$ having data type context $c$, $bes$ are the corresponding being predicted expressions, $types(bes)$ determines the set of the data type of the tokens in $bes$.

For each kind of context, for each case, we investigate if every  data type in $types(bes)$ can be found in any other cases having the same context in different methods or files.

%
The results are shown in Tab.~\ref{type_explore}, where $types(bes)$ determines the set of the data type of the tokens in the being predicted expressions $bes$. The results show that . That means...


\begin{definition} [Program type rules]

\end{definition}

\begin{definition}[Valid candidates] 
Given a excode sequence $S = e_1e_2...e_n$, the vocabulary $\mathscr{V}$, and a set of program rule $R$, the set of valid excode token candidates $C$ is the set of tokens $C = \bigcap_{r \in R} r(S)$.
\end{definition}


\textbf{The intuition of type rules}

%\begin{definition} [Accessibility rule] 
%Accessible elements
%\end{definition}



Example:

\input{type_exploratory}
